Multi-level Distance Regularization for Deep Metric Learning

We propose a novel distance-based regularization method for deep metric learning called Multi-level Distance Regularization (MDR). MDR explicitly disturbs a learning procedure by regularizing pairwise distances between embedding vectors into multiple levels that represents a degree of similarity between a pair. In the training stage, the model is trained with both MDR and an existing loss function of deep metric learning, simultaneously; the two losses interfere with the objective of each other, and it makes the learning process difficult. Moreover, MDR prevents some examples from being ignored or overly influenced in the learning process. These allow the parameters of the embedding network to be settle on a local optima with better generalization. Without bells and whistles, MDR with simple Triplet loss achieves the-state-of-the-art performance in various benchmark datasets: CUB-200-2011, Cars-196, Stanford Online Products, and In-Shop Clothes Retrieval. We extensively perform ablation studies on its behaviors to show the effectiveness of MDR. By easily adopting our MDR, the previous approaches can be improved in performance and generalization ability.

==> section/figure/figure3.tex <==
		
% \begin{figure*}[t!]
% 	\begin{center}
% 			\includegraphics[width=12cm]{images/figure5.pdf}
% 	\end{center}
% 	\vspace{-0.3cm}
% 	\caption{ 
% 	Ablation studies for the initial configuration of levels and the hyper-parameter $\lambda$ on CUB-200 \cite{CUB-200}; we experiment on seven configurations while varying the $\lambda$ from $0$ to $1$, and report the Recall@1 on the test set.
% 	The values inside $\{\dots\}$ are the initial values of each level in $\mathcal{S}$. 
%     }
% 	\label{fig:ablation}
% \vspace{-0.6cm}
% \end{figure*}

		

